Towards Optimizing Human-Centric Objectives in AI-Assisted Decision-Making With Offline Reinforcement Learning

Imagine if AI decision-support tools not only complemented our ability to make accurate decisions, but also improved our skills, boosted collaboration, and elevated the joy we derive from our tasks. Despite the potential to optimize a broad spectrum of such human-centric objectives, the design of current AI tools remains focused on decision accuracy alone. We propose offline reinforcement learning (RL) as a general approach for modeling human-AI decision-making to optimize human-AI interaction for diverse objectives. RL can optimize such objectives by tailoring decision support, providing the right type of assistance to the right person at the right time. We instantiated our approach with two objectives: human-AI accuracy on the decision-making task and human learning about the task and learned decision support policies from previous human-AI interaction data. We compared the optimized policies against several baselines in AI-assisted decision-making. Across two experiments (N=316 and N=964), our results demonstrated that people interacting with policies optimized for accuracy achieve significantly better accuracy -- and even human-AI complementarity -- compared to those interacting with any other type of AI support. Our results further indicated that human learning was more difficult to optimize than accuracy, with participants who interacted with learning-optimized policies showing significant learning improvement only at times. Our research (1) demonstrates offline RL to be a promising approach to model human-AI decision-making, leading to policies that may optimize human-centric objectives and provide novel insights about the AI-assisted decision-making space, and (2) emphasizes the importance of considering human-centric objectives beyond decision accuracy in AI-assisted decision-making, opening up the novel research challenge of optimizing human-AI interaction for such objectives.

==> sections/intro-v3.tex <==
\section{Introduction}

%[[help -- the intro is not in an acceptable shape]]

%motivating question, problem importance
AI is playing an increasingly influential role in assisting decision-makers across critical domains, ranging from healthcare to social welfare to finance~\cite{bannon2023when, gaube2021ai, kawakami2022improving, lee2019webuildai}. This AI assistance is typically comprised of a decision recommendation, prediction or a risk score accompanied by an explanation that is intended to help decision-makers understand the reason behind and discern the quality of AI's recommendation (we will refer to this approach as simple explainable AI or SXAI). A critical objective is to achieve human-AI complementarity, where the joint human and AI accuracy in decision-making outperforms that of either alone. However, this remains a significant challenge and an active area of research~\cite{bansal2021does, bucinca2021trust, ma2023should, noti2022learning, hemmer2021complement, vasconcelos2023explanations}.
%While such AI assistance is widespread, a critical objective of achieving human-AI complementarity, where the joint human and AI accuracy in decision-making outperforms that of either alone, remains a significant challenge and an active area of research~\cite{bansal2021does, bucinca2021trust, ma2023should, noti2022learning, hemmer2021complement, vasconcelos2023explanations}. 
We contend that the lack of human-AI complementarity is partly due to the design of current AI decision-support tools: these generally provide a fixed type of support (i.e., SXAI) regardless of the specific decision, person, or broader context. Meanwhile, alternative human-AI interaction approaches are being developed (e.g., cognitive forcing~\cite{bucinca2021trust}, evaluative AI~\cite{miller2023evaluative}, self explanation~\cite{danry2023don}, explanation without decision recommendation~\cite{gajos2022people}), and there is growing evidence that the choice of the optimal human-AI interaction approach depends on multiple contextual factors, including factors specific to a decision instance (such as a person's knowledge and confidence related to particular a decision instance) as well as AI's confidence~\cite{noti2022learning}. However, we do not yet have fully systematized knowledge to indicate what type of interaction should be presented under what circumstances.


% Meanwhile, evidence indicates that in human-AI decision-making, the effectiveness of different human-AI interaction approaches varies significantly with individual differences and contextual factors. Factors such as a person's willingness to engage cognitively with AI, the difficulty of the particular decision instance, AI's uncertainty, and the decision-maker's expertise and confidence in a specific task are all important in determining human's cognitive engagement with and reliance on the AI, and the ultimate decision accuracy of the human-AI dyad.

% Further, as people increasingly interact with and incorporate AI suggestions into their workflow, optimizing objectives beyond decision accuracy will become more and more critical to the design of decision-support tools. For instance, research suggests that augmenting people's capabilities on tasks they carry out not only improves well-being~\cite{} and job satisfaction but also leads to greater productivity and long-term economic growth~\cite{}. As such, some human-centric objectives towards AI-powered decision-support tools that augment humans~\cite{siddarth2021ai}, may include optimizing for decision-makers' long-term learning, their skill improvement over time, or their task enjoyment. 


Further, the anticipated large-scale deployment of AI-powered decision aids is likely to transform many jobs. There are moral and economic reasons to look for ways to deploy these technologies in a manner that complements workers and enhances their abilities, rather than diminish their roles or replace them without offering new opportunities~\cite{acemoglu2023can, siddarth2021ai}. However, many of the current deployments of AI-powered decision support systems are likely to negatively alter the existing workplace dynamics. For example, when workers rely on one another for help with difficult decisions, such help typically results in \em incidental learning \em that enables workers to develop their skill over time~\cite{berlin1992consultants}. In fact, some researchers argue that a large fraction of learning that occurs in organizations happens via informal channels such as incidental learning~\cite{marsick01:informal,marsick2017rethinking} and such learning is essential not just for workforce development but also for worker well-being~\cite{deci2017self}. However, receiving help from systems that offer a decision recommendation accompanied by an explanation does not seem to result in incidental learning~\cite{gajos2022people}. Instead, it can lead workers to incorrectly increase their confidence in their ability to perform similar tasks in the future~\cite{fisher2021knows,fisher2021harder}. %Thus, the currently popular explainable AI designs critically rely on knowledgeable workforce to supervise the performance of the algorithms but a large scale deployment of such systems is likely to lead to a reduction of skill in the workforce, while simultaneously making the workers more overconfident in their (dwindling) abilities. 
Thus, we argue that worker skill development should be one of the objectives in the design of decision support systems alongside improving the quality, efficiency, and consistency of decision-making.



%what is our approach
 
Considering the importance of context and diverse objectives in AI-assisted decision-making, AI support needs to be dynamic, changing in response to context for optimizing specified objectives like decision accuracy or human learning. But how to decide which kind of AI assistance is best for whom and when? In this paper, we propose a reinforcement learning (RL) based approach for providing such adaptive support to decision-makers. RL is a particularly appealing approach for modeling human-AI decision-making dynamics due to its ability to capture nuanced contextual factors as part of the state space, model objectives that are sparse or harder to capture (like human learning) as part of the reward, and adapt the support with an action space comprised of different types of AI support effective for specific contexts. Central to our proposed approach is the use of \em offline \em RL to derive optimal support policies from existing datasets of human-AI decisions with various AI assistance. This offers a safer alternative to real-time exploration which may pose significant risks or incur high costs in actual human-AI decision-making settings.

To instantiate our RL-based adaptive support approach, we considered two objectives: (1) decision \em accuracy \em, and (2) \em human learning \em about the task domain, as a human-centric objective we may seek to optimize in AI-assisted decision-making. Drawing insights from prior work about the effectiveness of different assistance for the two objectives in question~\cite{bucinca2021trust, gajos2022people}, we constructed an action space with four AI assistance types: \em no assistance\em, \em AI recommendation and explanation (i.e., SXAI)\em, \em explanation only \em and \em assistance on demand\em. We modeled the state space to account for factors that may require tailored AI assistance to achieve these objectives. One key factor is the individual's Need for Cognition (NFC), a stable personality trait indicating a person's inclination towards cognitively demanding activities, which affects engagement with AI support~\cite{gajos2022people, bucinca2021trust}. Additionally, the state space includes AI's uncertainty, the individual's knowledge of the decision instance, and overall task proficiency: all of these influence the effectiveness of different AI support types.

We broadly hypothesized that (1) people with different levels of NFC would benefit from different types of AI support for objectives that require cognitive engagement (\em i.e.\em, learning), (2) people interacting with optimized policies would outperform or perform as well as those interacting with policies that do not account for contextual factors, and would outperform people interacting with policies optimized for the other objectives.

%what are our results
To explore these hypotheses, we first conducted a data collection study with an exploratory policy (N = 142), in which the type of AI support was uniformly sampled in each decision instance. From the collected data, we learned optimal policies for the two objectives (immediate decision-making accuracy and learning) separately for individuals with high and low NFC. Our analysis of the distribution of types of AI assistance is in line with our current understanding of the human-AI decision-making space and reveals that the optimal policies are significantly different, in meaningful ways, for different objectives and different NFC groups. Examining the policies further led to discovering new insights about the AI-assisted decision-making space. Specifically, we discovered that participants low in NFC are unlikely to request AI assistance when that assistance is offered on demand.

To evaluate the effectiveness of the learned policies, we carried out two separate experiments. In both experiments, we compared how well participants performed on specific objectives (i.e., accuracy and learning) when they used the optimal policies versus when they used various baseline methods and policies that were optimized for a different objective.
Our results from the first (N=316) and second (N=964) experiment demonstrated that policies that are optimized for accuracy consistently, and significantly improved the immediate decision accuracy of both NFC groups compared to various baselines and learning-optimized policies.  Notably, participants high in NFC (in Experiment 1) and participants low in NFC (in Experiment 2) achieved complementary human-AI team performance with the accuracy-optimized policy, outperforming both human and AI accuracy alone on the task.  Our results showed that learning as an objective was more challenging to optimize for compared to immediate decision accuracy. %Specifically, in our first experiment individuals low in NFC interacting with the learning policy learned significantly more than individuals low in NFC interacting with the accuracy policy. In the second experiment, however, the same two policies were not significantly different from one another for the learning outcome. We partly attribute the weakness of the learning signal to reduced exposure to concepts and opportunities to learn and more broadly to the difficulty of the task and explanation design.

Delving into mechanisms that drive accuracy and learning in AI-assisted decision-making, we investigated the connection between overreliance and cognitive engagement (measured through learning outcomes). Challenging the common assumption that overreliance arises from limited cognitive engagement, we observed that for low NFC participants, the policy that led to the most learning also resulted in the highest overreliance on AI.

%implications
Together, our results demonstrate that AI support in decision-making needs to be dynamic, and that offline RL is a powerful approach for modeling the dynamics of human-AI decision-making. It can lead to policies that significantly optimize specific objectives, as well as leading to new insights about the human-AI decision-making space from interpreting the learned policies. 
Separately, our results also demonstrate that overreliance on AI may stem from various factors. It may be a result of superficial engagement with AI-provided assistance, but it may also be due to people engaging with the provided assistance \em and \em finding the AI's (misleading) explanation plausible. Understanding these nuances is essential for developing effective human-AI interaction techniques that promote appropriate reliance and enhance learning.
More broadly, with AI increasingly shaping the workplace, our work emphasizes the importance of incorporating human-centric objectives, such as learning about the task domain, when designing AI for decision support. Our work opens up a novel research challenge of designing novel explanations and human-AI interaction techniques that optimize human-centric objectives along with decision accuracy in AI-assisted decision-making.

% In summary, this paper makes the following contributions:

% \begin{itemize}
%     \item We introduce and illustrate the potential of offline RL as a promising method for modeling the complexities of human-AI decision-making, allowing the development of personalized decision-support policies that optimize different objectives while accommodating individual differences and other relevant contextual factors.
%     \item We demonstrate the potential of offline RL as a means to discover insights about the AI-assisted decision-making space.
%     \item We contribute new evidence demonstrating the significance of individual differences in cognitive motivation (i.e., Need for Cognition), as a factor to be taken into account when designing AI systems for decision support.
%     \item We demonstrate that overreliance on AI does not necessarily indicate a lack of cognitive engagement.

%We further show that cognitive engagement may not necessarily come at the cost of negative subjective experience in AI-assisted decision-making.

% \end{itemize}

%what are the implications of our results


%% emphasize cognitive engagement and reliance 

%%%one of the key objectives, a key objective there could exist

%% NFC is a dimension that we chose, one could pick other traits. We just focus on NFC on this paper



==> sections/intro-v4.tex <==
\section{Introduction}


Imagine AI decision-support tools that not only complement our ability to make accurate decisions, but also improve our skills, boost efficiency, and elevate the joy we derive from our tasks. Such human-centric objectives seem unattainable with the current decision-support tools, which have been consistently shown to hinder objectives such as human-AI complementarity in decision accuracy and recently also to hamper human skill improvement in the task. We contend that this limitation is partly due to the design of current AI decision-support tools: these generally provide a \textit{fixed} type of support –- an AI recommendation and an explanation -- regardless of the specific decision, person, or broader context. %For example, although research has shown people’s propensity to overrely on wrong AI suggestions, current decision support offers AI recommendations, even when the underlying model has high uncertainty. Further, recent evidence suggests some human-AI interaction techniques (AI explanations without recommendation) lead to increased cognitive engagement which may be beneficial for optimizing human skills on the task but may add cognitive effort if an individual is already skilled. 
However, such support may not always be ideal across objectives and contexts as previous work has shown people do not engage cognitively with AI information when recommendations are provided and to rely on the AI. As such, for accuracy as the objective, we may choose not to provide people with AI recommendations when the AI is uncertain about the decision which may lead the person astray. Or when optimizing human learning, we may choose to compel people to cognitively engage with AI support only at instances when they would learn.
While there are novel human-AI interaction approaches being developed and there is growing evidence that the choice of the optimal human-AI interaction approach depends on multiple contextual factors, including factors specific to a decision instance (such as a person's knowledge and confidence related to particular a decision instance), individual differences in motivation to think~\cite{bucinca2021trust, gajos2022people}, as well as AI's confidence~\cite{noti2022learning}, we do not yet have fully systematized knowledge to indicate what type of interaction should be presented under what circumstances.

Considering the importance of context and diverse objectives in AI-assisted decision-making, we argue AI support needs to be dynamic, changing in response to context for optimizing specified human-centric objectives like human-AI complementarity in decision accuracy or human learning. But how to decide which kind of AI assistance is best for whom and when? In this paper, we propose casting the problem of human-AI decision-making as a Markov Decision Process and applying reinforcement learning (RL) algorithms for learning policies that adaptively present different types of AI assistance in each decision instance, while optimizing different interaction objectives. RL is a particularly appealing approach for modeling human-AI decision-making dynamics due to its ability to capture nuanced contextual factors as part of the state space, model objectives that are sparse or harder to capture (like human learning or task enjoyment) as part of the reward, and adapt the support with an action space comprised of different types of human-AI interaction techinques effective for specific contexts. Central to our proposed approach is the use of \em offline \em RL to derive optimal support policies from existing datasets of human-AI decisions with various AI assistance, as a safer alternative to real-time exploration which may pose significant risks or incur high costs in actual human-AI decision-making settings (e.g., clinical setting).

We instantiate our RL-based adaptive support approach, by considering two objectives: (1) decision \em accuracy \em, and (2) \em human learning \em about the task domain, as human-centric objectives we may seek to optimize in AI-assisted decision-making and as examples of dense (accuracy) and sparse rewards (learning) in our proposed approach. Drawing insights from prior work about the effectiveness of different assistance for the two objectives in question~\cite{bucinca2021trust, gajos2022people}, we constructed an action space with four AI assistance types: \em no assistance\em, \em AI recommendation and explanation\em, \em explanation only \em and \em assistance on demand\em. We modeled the state space to account for factors that may require tailored AI assistance to achieve these objectives. One key factor is the individual's Need for Cognition (NFC), a stable personality trait indicating a person's inclination towards cognitively demanding activities, which affects engagement with AI support~\cite{gajos2022people, bucinca2021trust}. Additionally, the state space includes AI's uncertainty, the individual's knowledge of the decision instance, and overall task proficiency: all of these influence the effectiveness of different AI support types. We first conducted a data collection study with an exploratory policy (N = 142), in which the type of AI support was uniformly sampled in each decision instance. From the collected data, we learned optimal policies for the two objectives (immediate decision-making accuracy and learning). To evaluate the effectiveness of the learned policies, we carried out two separate experiments in which we compared the learned policies with several baselines.

%We broadly hypothesized that (1) people interacting with optimized policies would outperform or perform as well as those interacting with policies that do not account for contextual factors, and would outperform people interacting with policies optimized for the other objectives and (2) people with different levels of NFC would benefit from different types of AI support for objectives that require cognitive engagement (\em i.e.\em, learning). To explore these hypotheses, % We found evidence for our hypotheses in interpreting the distributions of actions (types of AI assistance) the policies had learned and through the evaluation studies.

Our results demonstrate that AI support in decision-making needs to be dynamic, and that offline RL is a powerful approach for modeling the dynamics of human-AI decision-making. It can lead to policies that significantly optimize specific objectives, as well as leading to discovery of new insights about the human-AI decision-making space from interpreting the learned policies.  
First, our analysis of policies aligns with current understanding of the human-AI decision-making space, showing that optimal AI assistance policies vary significantly across different objectives and NFC groups. Further examination of the policies led to uncovering new insights about AI-assisted decision-making (that participants with low NFC are less likely to seek on-demand AI assistance). Second, in both evaluation experiments, we compared how well participants performed on specific objectives (i.e., accuracy and learning) when they used the optimal policies versus when they used various baseline methods and policies that were optimized for a different objective. Our results from the first (N=316) and second (N=964) experiments demonstrated that policies that are optimized for accuracy consistently, and significantly improved the immediate decision accuracy of both NFC groups compared to various baselines and learning-optimized policies. Our results showed that learning as an objective was more challenging to optimize for compared to immediate decision accuracy.










==> sections/intro-v5.tex <==
\section{Introduction}

Imagine AI decision-support tools that not only complement our ability to make accurate decisions, but also improve our skills, boost efficiency, and elevate the joy we derive from our tasks. With aspiration of designing human-centric decision-support tools, we propose a general approach for modeling human-AI decision-making and present preliminary evidence of its promise to optimize such human-centric objectives. Our approach seeks to optimize different objectives by learning policies that adaptively provide decision support to humans — the right type of assistance, to the right person, at the right time. For example, rather than showing AI recommendation and explanations for each decision task, when optimizing decision accuracy, our policies learn to withhold AI recommendations when the AI is uncertain so that the human does not overrely on it. When seeking to optimize human skills, they learn to show only partial support (i.e., explanation only) so people cognitively engage to arrive at the decision recommendation themselves. Or they learn to provide more engaging AI support to people who are more likely to superficially engage with AI provided information.

To enable such adaptive AI support, we cast the problem of human-AI decision-making as a Markov Decision Process and learn policies that optimize different objectives with offline reinforcement learning (RL). We propose RL as a particularly appealing approach for optimizing human-centric objectives in AI-assisted decision-making due to its ability to model objectives that are sparse or harder to capture (like human learning or task enjoyment) as part of the reward, to capture human-centric and contextual factors (e.g., human's skill, load, motivation, AI's uncertainty) as part of the state space, and adapt the support with an action space comprised of different types of human-AI interaction techniques effective for specific contexts. Central to our proposed approach is the use of \em offline \em RL to derive optimal support policies from existing datasets of human-AI decisions with various AI assistance, as a safer alternative to real-time exploration which may pose significant risks or incur high costs in actual human-AI decision-making settings (e.g., clinical setting).


Our proposed approach is highly customizable with the potential to optimize various objectives in AI-assisted decision-making -- including accuracy, human skill improvement, time, enjoyment, or the cost of assistance -- by appropriately crafting the reward and constructing the state and action spaces. For this paper, we focus on optimizing \em accuracy \em and \em human learning \em about the task as objectives we may seek to optimize in AI-assisted decision-making and as examples of dense (accuracy) and sparse rewards (human learning) in our proposed approach. Drawing insights from prior work about the effectiveness of different assistance for the two objectives in question~\cite{bucinca2021trust, gajos2022people}, we constructed an action space with four AI assistance types: \em no assistance\em, \em AI recommendation and explanation\em, \em explanation only \em and \em assistance on demand\em.  We modeled the state space to account for human and contextual factors that may require tailored AI assistance to achieve these objectives. Our state space consisted of the concept in question, AI's uncertainty regarding the decision, alongside human-centric factors including individual's knowledge related to the decision, their overall task proficiency, and notably their Need for Cognition (NFC). NFC, a stable personality trait indicating a person's inclination towards cognitively demanding activities, plays a crucial role in determining how likely a person is to engage with AI support~\cite{gajos2022people, bucinca2021trust}, thereby influencing the effectiveness of different human-AI interaction techniques to achieve objectives that require cognitive engagement (e.g., human learning).

We first conducted a data collection study (N=142) in which participants made sequential decisions related to an exercise prescription task. In the data collection study participants interacted with an exploratory decision-supoprt policy that sampled AI assistance types uniformly.
From these interaction data, we applied Q-learning to learn policies that optimized accuracy (immediate accuracy on the task) and human learning (accuracy on post-intervention questions).
We conducted two types of evaluations of our approach: a computational evaluation of the optimized policies and two evaluation studies with human-subjects interacting with the optimized policies and various baselines. First, our computational analysis and interpretation of the learned policies revealed that optimal policies are different, in meaningful ways and in line with current understanding of the space, for different contexts and people with different Need for Cognition (NFC). Examining the policies further led to discovering new insights about the AI-assisted decision-making space. Specifically, we discovered that participants low in NFC are unlikely to request AI assistance when that assistance is offered on demand.
Second, our results from the first (N=316) and second (N=964) human-subject studies demonstrated that policies optimized for accuracy consistently, and significantly improved the immediate decision accuracy of both NFC groups compared to various baselines and learning-optimized policies. Whereas, learning-optimized policy led to significantly more learning than the accuracy-optimized policy only for the group low in NFC and only in the first experiment. Our results indicate that learning as an objective was more challenging to optimize for compared to immediate decision accuracy. We believe this is partially due to the weakness of the signal and the lack of actions (i.e., human-AI interaction techniques) that robustly improve learning.

Separately, our results present new findings in AI-assisted decision-making. Seeking to understand the effectiveness of different human-AI interaction techniques for optimizing learning and accuracy, we investigated the connection between overreliance (measured through reliance on wrong AI suggestions) and cognitive engagement (measured through learning outcomes). Our results showed that for participants low in NFC, the policy that led to the most learning (i.e., explanation only)  also resulted in the highest overreliance on AI. Thus, challenging the common assumption that overreliance arises from limited cognitive engagement, we demonstrated that people may overrely on the AI provided information even when they cognitively engage with it. We believe that overreliance is a consequence of a lack of \em critical \em engagement with AI support, which entails not only cognitively engaging with AI but also exercising critical judgment in integrating the provided information into decision-making processes.

%More broadly, with AI increasingly shaping the workplace, our work emphasizes the importance of incorporating human-centric objectives, such as learning about the task domain, when designing AI for decision support. Our work opens up a novel research challenge of designing novel explanations and human-AI interaction techniques that optimize human-centric objectives along with decision accuracy in AI-assisted decision-making.

In summary, this paper makes the following contributions:

 \begin{itemize}
     \item We introduce and illustrate the potential of offline RL as a promising method for modeling the complexities of human-AI decision-making, allowing the development of decision-support policies that optimize human-centric objectives in AI assisted decision-making.
    \item We demonstrate the potential of offline RL as a means to discover insights about the AI-assisted decision-making space.
     \item We contribute new evidence demonstrating the significance of individual differences in cognitive motivation (i.e., Need for Cognition), as a factor to be taken into account when designing AI systems for decision support.
    \item We show that overreliance on AI does not necessarily indicate a lack of cognitive engagement.
     \item Our instantiation of the proposed approach is consistently successful in improving joint human-AI accuracy, achieving even human-AI complementarity, but only partially successful in improving human learning.
    \item Our work opens up a novel research challenge of designing novel explanations and human-AI interaction techniques that optimize learning and other human-centric objectives along with decision accuracy in AI-assisted decision-making.

%We further show that cognitive engagement may not necessarily come at the cost of negative subjective experience in AI-assisted decision-making.

 \end{itemize}


%where the objective of the human-AI decision-making (e.g., accuracy, skill improvement, task enjoyment) is the reward of the RL agent. The state is constructed by relevant contextual factors, including factors specific to a decision instance (such as a person's knowledge and confidence related to particular a decision instance), individual differences in motivation to think~\cite{bucinca2021trust, gajos2022people}, as well as AI's confidence~\cite{noti2022learning}. And the action space is comprised of human-AI interaction techniques that may be effective for specific contexts or specific objectives, such as providing people with AI decision recommendations and explanations, explanations with no recommendations, or not providing them with any assistance.

%While there are novel human-AI interaction approaches being developed and there is growing evidence that the choice of the optimal human-AI interaction approach depends on multiple contextual factors, including factors specific to a decision instance (such as a person's knowledge and confidence related to particular a decision instance), individual differences in motivation to think~\cite{bucinca2021trust, gajos2022people}, as well as AI's confidence~\cite{noti2022learning}, we do not yet have fully systematized knowledge to indicate what type of interaction should be presented under what circumstances. Our research demonstrates that AI support in decision-making needs to be dynamic, and that offline RL is a powerful approach for modeling the dynamics of human-AI decision-making. It can lead to policies that significantly optimize specific objectives, as well as leading to new insights about the human-AI decision-making space from interpreting the learned policies. 

==> tables/subjective_measures_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\begin{tabular}{l|l|l|lll|l}
                                                                                         &                                                                                 & \multicolumn{1}{c|}{}                                                & \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ (Standard Error)\end{tabular}}}                                                                                                                                                                                           & \multicolumn{1}{c}{}                                        \\ \cline{4-6}
\multirow{-2}{*}{}                                                                       & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}NFC \\ group\end{tabular}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Post-hoc analyses}}}    & \multicolumn{1}{l|}{\textbf{SXAI}}                                                                 & \multicolumn{1}{l|}{\textbf{accuracy}}                                                             & \textbf{learning}                                                             & \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Significance}}} \\ \hline
                                                                                         & \textit{low}                                                                    & \{learning, SXAI, accuracy\}                                         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}3.33\\ (0.16)\end{tabular}}                         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}3.31\\ (0.15)\end{tabular}}                         & {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}3.56\\ (0.14)\end{tabular}}  & {\color[HTML]{343434} $F_{2, 141} = 0.40, n.s.$}            \\
\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Perceived \\ learning\end{tabular}}} & \cellcolor[HTML]{EFEFEF}\textit{high}                                           & \cellcolor[HTML]{EFEFEF}\{accuracy, SXAI, learning\}                 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}3.66\\ (0.13)\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}3.68\\ (0.14)\end{tabular}} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}3.48\\ (0.12)\end{tabular} & \cellcolor[HTML]{EFEFEF}$F_{2, 171} = 0.48,  p = n.s.$      \\ \hline
                                                                                         & \textit{low}                                                                    & \{learning, accuracy, SXAI\}                                         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}3.33\\ (0.17)\end{tabular}}                         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}3.35\\ (0.16)\end{tabular}}                         & \begin{tabular}[c]{@{}l@{}}3.50\\ (0.16)\end{tabular}                         & {\color[HTML]{343434} $F_{2, 141} = 0.70, n.s.$}            \\
\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Task \\ enjoyment\end{tabular}}}     & \cellcolor[HTML]{EFEFEF}\textit{high}                                           & \cellcolor[HTML]{EFEFEF}\{accuracy, SXAI, learning\}                 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}3.54\\ (0.14)\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}3.62\\ (0.16)\end{tabular}} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}3.35\\ (0.14)\end{tabular} & \cellcolor[HTML]{EFEFEF}$F_{2, 171} = 0.41,  p = n.s.$      \\ \hline
                                                                                         & \textit{low}                                                                    & \{SXAI, learning, accuracy\}                                         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}2.98\\ (0.17)\end{tabular}}                         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}2.88\\ (0.15)\end{tabular}}                         & \begin{tabular}[c]{@{}l@{}}2.90\\ (0.16)\end{tabular}                         & {\color[HTML]{343434} $F_{2, 141} = 0.09, n.s.$}            \\
\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Mental \\ demand\end{tabular}}}      & \cellcolor[HTML]{EFEFEF}\textit{high}                                           & \cellcolor[HTML]{EFEFEF}\{SXAI, accuracy, learning\}        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}3.08\\ (0.14)\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}2.94\\ (0.15)\end{tabular}} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}2.80\\ (0.14)\end{tabular} & \cellcolor[HTML]{EFEFEF}$F_{2, 171} = 0.344,  n.s.$         \\ \hline
                                                                                         & \textit{low}                                                                    & \textbf{\{learning\} \textgreater \{SXAI\}}                          & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}3.09\\ (0.15)\end{tabular}}                         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}3.51\\ (0.14)\end{tabular}}                         & \begin{tabular}[c]{@{}l@{}}3.56\\ (0.14)\end{tabular}                         & {\color[HTML]{343434} $F_{2, 141} = 3.12,  p = .05$}        \\
\multirow{-2}{*}{\textbf{Trust}}                                                         & \cellcolor[HTML]{EFEFEF}\textit{high}                                           & \cellcolor[HTML]{EFEFEF}\textbf{\{accuracy\} \textgreater \{ SXAI\}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}3.19\\ (0.12)\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}3.76\\ (0.13)\end{tabular}} & \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}3.35\\ (0.12)\end{tabular} & \cellcolor[HTML]{EFEFEF}$F_{2, 171} = 5.52,  p = .001$     
\end{tabular}
\caption{Results of subjective measures. Differences indicated by > symbol are statistically significant. Conditions that share brackets do not differ significantly. Missing conditions do not differ significantly from either group.}
\label{tbl:subjective-measures}
\end{table}
